ScoreShield: Differentially Private Release of Similarity Scores

A growing number of applications, such as biometrics and retrieval-augmented generation (RAG), rely on cosine similarity scores computed between vector embeddings of text, images, or audio. These systems return similarity scores through their APIs for ranking and verification. However, such releases can leak information about individual records and enable membership inference attacks. While differential privacy (DP) provides a principled metric for quantifying attack risks, na\"ive application of DP mechanisms---such as adding i.i.d. Gaussian noise to vector entries---leads to excessive distortion (i.e., low utility) at a given privacy constraint that scales poorly with the number of released scores. We propose \textsc{ScoreShield}, a perturb-then-project mechanism that adds Gaussian noise calibrated to global sensitivity of the chosen score release regime and then projects the result onto the feasibility set of valid cosine objects. \textsc{ScoreShield} satisfies $(\varepsilon,\delta)$-DP for releasing similarity score vectors and Gram matrices. We provide utility guarantees for the exact Frobenius metric projection used in the risk analysis, and prove convergence to feasibility for the practical averaged alternating-projection solver used for large-scale Gram releases. For full pairwise cosine Gram release under record-level replacement adjacency, the exact-projection bound improves the $n$-dependence of squared Frobenius risk from $\Theta(n^3)$ for the na\"ive Gaussian baseline to $\mathcal{O}(n^2)$ for fixed privacy parameters, with sharper local bounds at low-rank Grams. We evaluate the mechanism across RAG, face recognition, semantic retrieval, image similarity, and recommender-system tasks.

==> appx_results/case1/results_ir101.tex <==
\begin{tabular}{cccccccccccccc}
\toprule
$\varepsilon$ & $\delta$ & val/IJBC_gt_aligned/Norm:True_Det:False_tpr_at_fpr_1e-06 & val/IJBC_gt_aligned/Norm:True_Det:False_tpr_at_fpr_1e-05 & val/IJBC_gt_aligned/Norm:True_Det:False_tpr_at_fpr_0.0001 & val/IJBB_gt_aligned/Norm:True_Det:False_tpr_at_fpr_1e-06 & val/IJBB_gt_aligned/Norm:True_Det:False_tpr_at_fpr_1e-05 & val/IJBB_gt_aligned/Norm:True_Det:False_tpr_at_fpr_0.0001 & val/agedb_30/acc & val/calfw/acc & val/cfpfp/acc & val/cplfw/acc & val/lfw/acc & Avg \\
\midrule
100.00 & 1e-7 & 58.54 & 72.81 & 83.41 & 25.60 & 65.13 & 79.26 & 75.72 & 80.02 & 79.34 & 76.77 & 87.57 & 71.29 \\
100.00 & 1e-6 & 68.08 & 77.37 & 85.49 & 28.39 & 70.83 & 82.23 & 77.15 & 81.85 & 81.24 & 76.53 & 88.55 & 74.34 \\
100.00 & 1e-5 & 70.31 & 80.71 & 87.98 & 32.37 & 73.99 & 84.81 & 78.47 & 82.77 & 82.41 & 79.25 & 90.37 & 76.68 \\
100.00 & 1e-4 & 73.18 & 83.68 & 89.87 & 29.36 & 76.48 & 86.85 & 79.78 & 84.47 & 84.73 & 80.10 & 92.05 & 78.23 \\
100.00 & 1e-3 & 79.99 & 87.05 & 91.82 & 26.29 & 81.09 & 89.16 & 82.65 & 86.13 & 87.01 & 82.63 & 93.87 & 80.70 \\
100.00 & 1e-2 & 80.47 & 88.73 & 93.08 & 31.80 & 83.32 & 90.57 & 85.72 & 89.20 & 89.56 & 84.35 & 96.03 & 82.98 \\
100.00 & 0.10 & 86.35 & 90.88 & 94.32 & 29.66 & 85.65 & 92.20 & 88.70 & 91.77 & 92.71 & 87.48 & 98.12 & 85.26 \\
100.00 & 0.20 & 86.26 & 91.42 & 94.71 & 39.36 & 86.00 & 92.57 & 90.43 & 92.63 & 93.91 & 88.40 & 98.70 & 86.76 \\
100.00 & 0.40 & 88.17 & 92.07 & 94.86 & 43.25 & 87.72 & 92.92 & 91.83 & 93.33 & 95.27 & 89.92 & 99.17 & 88.05 \\
100.00 & 0.60 & 87.92 & 92.33 & 95.15 & 35.69 & 87.37 & 93.13 & 93.40 & 93.65 & 96.23 & 90.32 & 99.33 & 87.68 \\
100.00 & 0.80 & 88.81 & 92.25 & 95.26 & 39.64 & 87.97 & 93.35 & 93.88 & 94.38 & 96.59 & 91.12 & 99.53 & 88.44 \\
\midrule
70.00 & 1e-7 & 24.47 & 40.48 & 58.17 & 16.29 & 37.13 & 55.07 & 70.10 & 73.08 & 73.59 & 71.38 & 81.37 & 54.65 \\
70.00 & 1e-6 & 33.72 & 49.64 & 65.33 & 23.10 & 42.62 & 61.51 & 70.98 & 75.93 & 74.09 & 72.12 & 82.67 & 59.25 \\
70.00 & 1e-5 & 39.52 & 57.38 & 72.30 & 25.80 & 50.95 & 68.16 & 72.95 & 76.43 & 75.71 & 73.35 & 83.90 & 63.31 \\
70.00 & 1e-4 & 53.82 & 66.66 & 78.60 & 20.35 & 60.17 & 75.10 & 73.92 & 77.53 & 77.93 & 75.17 & 86.72 & 67.81 \\
70.00 & 1e-3 & 61.19 & 74.96 & 84.41 & 36.37 & 69.71 & 81.37 & 76.78 & 80.58 & 80.97 & 76.47 & 88.75 & 73.78 \\
70.00 & 1e-2 & 73.44 & 82.93 & 89.36 & 34.15 & 77.06 & 86.20 & 80.32 & 84.25 & 83.01 & 79.53 & 91.27 & 78.32 \\
70.00 & 0.10 & 81.22 & 88.55 & 92.73 & 27.91 & 82.78 & 90.05 & 84.72 & 87.87 & 88.57 & 83.72 & 95.55 & 82.15 \\
70.00 & 0.20 & 84.54 & 89.52 & 93.44 & 38.26 & 84.02 & 91.09 & 86.85 & 88.87 & 90.23 & 84.93 & 96.78 & 84.41 \\
70.00 & 0.40 & 85.97 & 90.91 & 94.30 & 44.22 & 85.58 & 91.85 & 89.35 & 90.98 & 92.73 & 86.72 & 97.82 & 86.40 \\
70.00 & 0.60 & 86.96 & 91.32 & 94.69 & 36.18 & 86.85 & 92.32 & 91.05 & 92.00 & 93.60 & 88.48 & 98.83 & 86.57 \\
70.00 & 0.80 & 87.40 & 91.92 & 94.87 & 38.26 & 86.93 & 92.78 & 91.95 & 93.53 & 95.29 & 89.25 & 99.20 & 87.40 \\
\midrule
35.00 & 1e-7 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 60.63 & 62.92 & 61.44 & 60.47 & 67.75 & 28.47 \\
35.00 & 1e-6 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 61.07 & 63.68 & 62.96 & 61.85 & 67.95 & 28.86 \\
35.00 & 1e-5 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 61.77 & 65.50 & 64.74 & 63.07 & 69.00 & 29.46 \\
35.00 & 1e-4 & 0.00 & 0.00 & 18.01 & 0.00 & 0.00 & 17.60 & 63.75 & 66.28 & 65.81 & 64.75 & 71.52 & 33.43 \\
35.00 & 1e-3 & 0.00 & 14.64 & 28.11 & 0.00 & 13.23 & 26.80 & 65.13 & 68.45 & 67.64 & 65.70 & 75.08 & 38.62 \\
35.00 & 1e-2 & 17.57 & 28.35 & 46.40 & 14.28 & 25.59 & 43.35 & 68.45 & 72.18 & 70.77 & 69.07 & 78.00 & 48.55 \\
35.00 & 0.10 & 42.13 & 58.61 & 73.00 & 26.07 & 52.52 & 69.58 & 72.73 & 77.13 & 76.34 & 73.43 & 84.23 & 64.16 \\
35.00 & 0.20 & 55.13 & 69.57 & 80.58 & 37.11 & 62.14 & 76.80 & 75.17 & 79.05 & 78.46 & 75.77 & 86.53 & 70.57 \\
35.00 & 0.40 & 69.21 & 79.14 & 87.12 & 30.30 & 73.36 & 84.23 & 78.65 & 82.52 & 81.96 & 78.17 & 89.68 & 75.85 \\
35.00 & 0.60 & 76.71 & 83.74 & 89.88 & 24.63 & 77.26 & 86.93 & 80.87 & 84.92 & 84.51 & 80.67 & 92.62 & 78.43 \\
35.00 & 0.80 & 77.07 & 86.53 & 91.85 & 35.02 & 81.17 & 88.79 & 83.07 & 86.52 & 86.64 & 82.63 & 94.22 & 81.23 \\
\midrule
30.00 & 1e-7 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 57.70 & 59.53 & 60.13 & 58.52 & 63.83 & 27.25 \\
30.00 & 1e-6 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 59.40 & 61.07 & 60.91 & 59.02 & 66.20 & 27.87 \\
30.00 & 1e-5 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 61.13 & 63.50 & 62.81 & 60.82 & 67.27 & 28.68 \\
30.00 & 1e-4 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 62.55 & 64.95 & 63.41 & 62.62 & 69.08 & 29.33 \\
30.00 & 1e-3 & 0.00 & 0.00 & 17.05 & 0.00 & 0.00 & 16.14 & 63.73 & 66.18 & 65.56 & 64.17 & 71.50 & 33.12 \\
30.00 & 1e-2 & 0.00 & 16.10 & 30.90 & 0.00 & 14.29 & 28.84 & 66.05 & 68.55 & 67.50 & 67.22 & 75.65 & 39.55 \\
30.00 & 0.10 & 27.65 & 41.93 & 60.11 & 19.44 & 38.86 & 56.23 & 70.57 & 73.98 & 71.77 & 70.80 & 81.65 & 55.73 \\
30.00 & 0.20 & 39.44 & 55.93 & 71.33 & 28.02 & 51.97 & 67.58 & 72.63 & 77.35 & 76.27 & 73.13 & 83.07 & 63.34 \\
30.00 & 0.40 & 54.00 & 70.91 & 81.70 & 36.80 & 65.96 & 78.37 & 74.38 & 79.47 & 78.23 & 75.15 & 87.50 & 71.13 \\
30.00 & 0.60 & 67.55 & 78.67 & 87.02 & 20.44 & 72.94 & 83.25 & 78.00 & 82.17 & 81.81 & 78.48 & 90.08 & 74.58 \\
30.00 & 0.80 & 74.49 & 83.36 & 90.06 & 31.31 & 77.54 & 86.76 & 79.72 & 84.47 & 84.71 & 80.62 & 92.18 & 78.66 \\
\midrule
25.00 & 1e-7 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 55.95 & 57.77 & 57.86 & 55.93 & 61.02 & 26.23 \\
25.00 & 1e-6 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 56.75 & 59.52 & 58.89 & 58.60 & 62.83 & 26.96 \\
25.00 & 1e-5 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 59.10 & 59.42 & 60.66 & 58.65 & 64.77 & 27.51 \\
25.00 & 1e-4 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 58.72 & 61.97 & 60.99 & 59.03 & 65.63 & 27.85 \\
25.00 & 1e-3 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 60.23 & 63.73 & 63.74 & 61.83 & 68.70 & 28.93 \\
25.00 & 1e-2 & 0.00 & 0.00 & 17.00 & 0.00 & 0.00 & 16.34 & 63.92 & 66.30 & 65.41 & 64.47 & 72.63 & 33.28 \\
25.00 & 0.10 & 12.80 & 24.78 & 41.07 & 11.58 & 21.43 & 38.88 & 67.53 & 70.53 & 70.04 & 67.85 & 78.02 & 45.86 \\
25.00 & 0.20 & 19.23 & 35.74 & 54.72 & 18.66 & 33.56 & 51.78 & 68.37 & 71.75 & 72.41 & 70.17 & 79.48 & 52.35 \\
25.00 & 0.40 & 40.68 & 55.13 & 71.30 & 25.35 & 50.67 & 66.89 & 72.15 & 75.65 & 75.61 & 72.50 & 83.57 & 62.68 \\
25.00 & 0.60 & 53.25 & 67.51 & 80.25 & 26.58 & 63.02 & 76.10 & 75.37 & 78.88 & 78.04 & 74.73 & 87.02 & 69.16 \\
25.00 & 0.80 & 64.33 & 76.95 & 85.64 & 34.54 & 69.76 & 82.26 & 77.58 & 81.00 & 80.40 & 77.17 & 89.08 & 74.43 \\
\midrule
20.00 & 1e-7 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 54.30 & 54.50 & 55.39 & 56.37 & 57.33 & 25.26 \\
20.00 & 1e-6 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 56.28 & 57.10 & 56.27 & 56.30 & 59.07 & 25.91 \\
20.00 & 1e-5 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 57.72 & 58.18 & 56.81 & 55.93 & 60.25 & 26.26 \\
20.00 & 1e-4 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 56.63 & 59.50 & 58.83 & 56.95 & 61.67 & 26.69 \\
20.00 & 1e-3 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 58.90 & 60.92 & 59.79 & 59.30 & 64.55 & 27.59 \\
20.00 & 1e-2 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 60.78 & 62.62 & 61.53 & 60.35 & 67.95 & 28.48 \\
20.00 & 0.10 & 0.00 & 0.00 & 20.15 & 0.00 & 0.00 & 19.95 & 63.87 & 67.82 & 67.16 & 64.87 & 72.97 & 34.25 \\
20.00 & 0.20 & 0.00 & 16.98 & 32.03 & 0.00 & 14.99 & 29.16 & 65.07 & 68.87 & 68.40 & 66.38 & 74.93 & 39.71 \\
20.00 & 0.40 & 18.99 & 31.37 & 50.28 & 13.84 & 29.79 & 46.65 & 68.88 & 71.35 & 71.83 & 70.13 & 79.78 & 50.26 \\
20.00 & 0.60 & 32.45 & 48.07 & 64.77 & 22.68 & 42.97 & 60.03 & 71.65 & 75.40 & 73.56 & 71.53 & 81.62 & 58.61 \\
20.00 & 0.80 & 45.84 & 61.56 & 75.12 & 29.11 & 56.03 & 72.10 & 73.05 & 77.35 & 75.96 & 73.90 & 85.17 & 65.93 \\
\midrule
15.00 & 1e-7 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 53.05 & 54.38 & 53.40 & 52.85 & 55.07 & 24.43 \\
15.00 & 1e-6 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 52.82 & 55.17 & 53.06 & 52.95 & 56.47 & 24.59 \\
15.00 & 1e-5 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 53.15 & 53.98 & 53.67 & 54.38 & 57.30 & 24.77 \\
15.00 & 1e-4 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 54.72 & 55.13 & 54.90 & 56.37 & 57.43 & 25.32 \\
15.00 & 1e-3 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 55.27 & 56.90 & 57.37 & 56.53 & 59.53 & 25.96 \\
15.00 & 1e-2 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 57.40 & 58.90 & 58.87 & 57.72 & 62.20 & 26.83 \\
15.00 & 0.10 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 61.37 & 62.82 & 61.96 & 60.37 & 67.02 & 28.50 \\
15.00 & 0.20 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 62.47 & 64.13 & 64.03 & 62.17 & 68.73 & 29.23 \\
15.00 & 0.40 & 0.00 & 0.00 & 22.47 & 0.00 & 0.00 & 21.60 & 64.25 & 67.48 & 67.36 & 64.82 & 73.43 & 34.67 \\
15.00 & 0.60 & 0.00 & 19.90 & 35.46 & 11.92 & 18.34 & 32.94 & 67.43 & 69.07 & 68.90 & 67.97 & 77.03 & 42.63 \\
15.00 & 0.80 & 16.10 & 31.52 & 49.03 & 11.43 & 28.21 & 46.55 & 68.78 & 71.92 & 71.81 & 70.37 & 79.12 & 49.53 \\
\midrule
N/A & N/A & 89.46 & 93.07 & 95.52 & 43.49 & 89.07 & 93.72 & 96.35 & 95.57 & 98.37 & 92.82 & 99.70 & 89.74 \\
\bottomrule
\end{tabular}


==> appx_results/case1/results_vitb.tex <==
\begin{tabular}{cccccccccccccc}
\toprule
$\varepsilon$ & $\delta$ & val/IJBC_gt_aligned/Norm:True_Det:False_tpr_at_fpr_1e-06 & val/IJBC_gt_aligned/Norm:True_Det:False_tpr_at_fpr_1e-05 & val/IJBC_gt_aligned/Norm:True_Det:False_tpr_at_fpr_0.0001 & val/IJBB_gt_aligned/Norm:True_Det:False_tpr_at_fpr_1e-06 & val/IJBB_gt_aligned/Norm:True_Det:False_tpr_at_fpr_1e-05 & val/IJBB_gt_aligned/Norm:True_Det:False_tpr_at_fpr_0.0001 & val/agedb_30/acc & val/calfw/acc & val/cfpfp/acc & val/cplfw/acc & val/lfw/acc & Avg \\
\midrule
100.00 & 1e-7 & 60.84 & 74.62 & 84.93 & 43.50 & 68.40 & 82.13 & 78.92 & 81.62 & 81.90 & 79.40 & 89.50 & 75.07 \\
100.00 & 1e-6 & 67.04 & 79.05 & 87.57 & 21.67 & 72.85 & 84.29 & 79.32 & 83.58 & 83.33 & 81.08 & 90.08 & 75.44 \\
100.00 & 1e-5 & 71.69 & 82.05 & 89.73 & 34.94 & 77.93 & 86.71 & 81.13 & 84.92 & 85.61 & 82.23 & 92.10 & 79.00 \\
100.00 & 1e-4 & 74.98 & 86.14 & 91.97 & 29.72 & 78.45 & 88.94 & 83.82 & 85.22 & 87.04 & 84.07 & 93.43 & 80.34 \\
100.00 & 1e-3 & 79.64 & 88.92 & 93.72 & 40.61 & 83.51 & 91.08 & 84.98 & 87.40 & 89.74 & 86.20 & 95.15 & 83.72 \\
100.00 & 1e-2 & 81.42 & 91.16 & 94.83 & 28.18 & 85.53 & 92.46 & 88.17 & 89.93 & 92.29 & 88.27 & 97.02 & 84.48 \\
100.00 & 0.10 & 82.59 & 92.89 & 95.78 & 32.69 & 87.83 & 94.01 & 91.30 & 92.58 & 95.46 & 90.82 & 98.78 & 86.79 \\
100.00 & 0.20 & 86.81 & 93.16 & 95.91 & 33.00 & 88.86 & 94.35 & 92.60 & 93.28 & 96.10 & 91.83 & 99.08 & 87.73 \\
100.00 & 0.40 & 86.18 & 93.60 & 96.33 & 38.83 & 89.40 & 94.72 & 93.83 & 94.52 & 97.31 & 92.95 & 99.42 & 88.83 \\
100.00 & 0.60 & 85.99 & 93.78 & 96.49 & 39.81 & 89.60 & 94.89 & 94.75 & 94.88 & 97.61 & 93.60 & 99.55 & 89.18 \\
100.00 & 0.80 & 84.34 & 94.06 & 96.56 & 36.83 & 90.22 & 95.15 & 95.68 & 95.33 & 98.10 & 94.10 & 99.70 & 89.10 \\
\midrule
70.00 & 1e-7 & 25.13 & 39.46 & 59.06 & 16.29 & 35.87 & 55.32 & 72.38 & 74.48 & 75.47 & 73.92 & 81.42 & 55.35 \\
70.00 & 1e-6 & 29.96 & 47.21 & 66.67 & 26.94 & 44.26 & 61.70 & 73.67 & 76.38 & 77.04 & 74.52 & 83.63 & 60.18 \\
70.00 & 1e-5 & 37.29 & 56.93 & 73.36 & 30.94 & 52.83 & 70.12 & 74.73 & 76.95 & 78.31 & 76.37 & 86.17 & 64.91 \\
70.00 & 1e-4 & 52.67 & 67.86 & 80.93 & 35.75 & 60.49 & 77.05 & 76.82 & 79.87 & 80.27 & 79.12 & 87.07 & 70.72 \\
70.00 & 1e-3 & 58.04 & 76.45 & 86.15 & 28.89 & 69.46 & 83.19 & 79.35 & 82.68 & 83.14 & 79.62 & 90.03 & 74.27 \\
70.00 & 1e-2 & 71.37 & 84.52 & 91.01 & 37.24 & 78.48 & 88.21 & 82.23 & 84.83 & 86.67 & 83.58 & 92.90 & 80.10 \\
70.00 & 0.10 & 81.20 & 90.44 & 94.31 & 27.32 & 85.10 & 92.04 & 86.47 & 89.50 & 90.69 & 87.67 & 95.85 & 83.69 \\
\midrule
35.00 & 1e-7 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 61.77 & 62.90 & 63.66 & 62.80 & 67.53 & 28.97 \\
35.00 & 1e-6 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 61.88 & 65.47 & 62.86 & 63.23 & 69.05 & 29.32 \\
35.00 & 1e-5 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 62.98 & 65.78 & 65.73 & 65.77 & 72.38 & 30.24 \\
35.00 & 1e-4 & 0.00 & 0.00 & 18.26 & 0.00 & 0.00 & 17.05 & 65.17 & 68.28 & 67.66 & 66.87 & 71.82 & 34.10 \\
35.00 & 1e-3 & 0.00 & 15.92 & 28.03 & 0.00 & 15.03 & 25.80 & 67.77 & 69.98 & 70.50 & 68.40 & 75.33 & 39.71 \\
35.00 & 1e-2 & 17.05 & 28.95 & 46.23 & 11.94 & 24.58 & 43.20 & 70.03 & 73.35 & 73.51 & 71.85 & 79.95 & 49.15 \\
35.00 & 0.10 & 43.42 & 57.97 & 74.08 & 21.27 & 53.43 & 71.02 & 75.63 & 77.98 & 79.03 & 76.55 & 86.35 & 65.16 \\
\midrule
30.00 & 1e-7 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 58.53 & 60.90 & 60.01 & 59.88 & 65.15 & 27.68 \\
30.00 & 1e-6 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 59.98 & 62.13 & 62.17 & 62.30 & 66.40 & 28.45 \\
30.00 & 1e-5 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 61.05 & 62.30 & 63.80 & 62.22 & 66.22 & 28.69 \\
30.00 & 1e-4 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 62.53 & 66.40 & 65.77 & 64.20 & 69.13 & 29.82 \\
30.00 & 1e-3 & 0.00 & 0.00 & 19.02 & 0.00 & 0.00 & 18.45 & 65.42 & 67.35 & 66.91 & 66.03 & 72.70 & 34.17 \\
30.00 & 1e-2 & 0.00 & 15.56 & 30.67 & 0.00 & 14.62 & 28.80 & 66.80 & 69.33 & 70.10 & 69.48 & 76.43 & 40.16 \\
30.00 & 0.10 & 25.75 & 41.70 & 60.18 & 16.35 & 36.54 & 56.38 & 71.95 & 75.13 & 75.69 & 73.88 & 82.95 & 56.05 \\
30.00 & 0.20 & 38.42 & 55.71 & 72.13 & 21.90 & 51.15 & 68.57 & 75.65 & 77.73 & 78.61 & 75.55 & 84.77 & 63.65 \\
30.00 & 0.40 & 59.83 & 72.27 & 83.74 & 30.84 & 66.40 & 80.69 & 78.22 & 81.27 & 81.97 & 79.60 & 88.68 & 73.05 \\
30.00 & 0.60 & 66.94 & 80.96 & 88.84 & 28.65 & 73.95 & 85.82 & 80.67 & 84.07 & 85.20 & 82.95 & 90.68 & 77.16 \\
30.00 & 0.80 & 73.60 & 85.86 & 91.46 & 22.94 & 79.55 & 88.96 & 82.27 & 86.55 & 87.44 & 83.52 & 93.28 & 79.58 \\
\midrule
25.00 & 1e-7 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 57.07 & 58.17 & 58.10 & 58.27 & 61.85 & 26.68 \\
25.00 & 1e-6 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 58.38 & 59.48 & 59.61 & 58.90 & 62.43 & 27.16 \\
25.00 & 1e-5 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 59.57 & 60.43 & 60.44 & 59.35 & 64.57 & 27.67 \\
25.00 & 1e-4 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 60.83 & 62.28 & 61.84 & 61.65 & 66.67 & 28.48 \\
25.00 & 1e-3 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 63.37 & 64.32 & 63.20 & 62.57 & 68.33 & 29.25 \\
25.00 & 1e-2 & 0.00 & 0.00 & 18.45 & 0.00 & 0.00 & 17.88 & 65.35 & 67.45 & 68.09 & 65.48 & 72.75 & 34.13 \\
25.00 & 0.10 & 14.24 & 23.08 & 40.62 & 12.96 & 20.93 & 38.62 & 69.53 & 72.35 & 72.54 & 70.85 & 78.50 & 46.75 \\
25.00 & 0.20 & 22.15 & 36.31 & 54.91 & 16.75 & 32.40 & 50.93 & 71.02 & 74.47 & 75.67 & 72.68 & 81.53 & 53.53 \\
25.00 & 0.40 & 41.10 & 56.44 & 72.11 & 27.59 & 50.54 & 68.34 & 74.12 & 77.57 & 76.59 & 76.27 & 85.32 & 64.18 \\
25.00 & 0.60 & 50.97 & 69.69 & 81.44 & 33.58 & 63.65 & 77.88 & 77.55 & 81.08 & 81.23 & 79.17 & 88.30 & 71.32 \\
25.00 & 0.80 & 65.19 & 78.83 & 87.55 & 25.03 & 72.02 & 84.03 & 79.85 & 82.85 & 83.23 & 80.92 & 90.25 & 75.43 \\
\midrule
20.00 & 1e-7 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 55.65 & 56.50 & 55.63 & 54.63 & 57.98 & 25.49 \\
20.00 & 1e-6 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 56.48 & 56.65 & 56.80 & 55.88 & 60.85 & 26.06 \\
20.00 & 1e-5 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 58.45 & 58.95 & 56.91 & 57.40 & 60.05 & 26.52 \\
20.00 & 1e-4 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 58.22 & 59.73 & 58.71 & 58.60 & 62.30 & 27.05 \\
20.00 & 1e-3 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 59.73 & 60.23 & 61.29 & 60.93 & 64.37 & 27.87 \\
20.00 & 1e-2 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 62.47 & 64.55 & 64.11 & 63.50 & 66.87 & 29.23 \\
20.00 & 0.10 & 0.00 & 0.00 & 20.40 & 0.00 & 0.00 & 19.77 & 65.18 & 69.18 & 68.61 & 67.00 & 73.47 & 34.87 \\
20.00 & 0.20 & 0.00 & 16.54 & 31.76 & 0.00 & 14.90 & 29.18 & 67.50 & 70.62 & 70.89 & 69.93 & 76.05 & 40.67 \\
20.00 & 0.40 & 18.79 & 32.46 & 50.77 & 15.71 & 29.11 & 47.32 & 70.87 & 72.52 & 73.14 & 72.72 & 80.30 & 51.25 \\
20.00 & 0.60 & 29.03 & 47.20 & 65.23 & 22.12 & 44.73 & 62.32 & 72.43 & 77.15 & 76.93 & 75.07 & 83.72 & 59.63 \\
20.00 & 0.80 & 44.87 & 62.17 & 76.83 & 28.01 & 56.69 & 72.87 & 76.42 & 78.83 & 79.03 & 76.63 & 86.67 & 67.18 \\
\midrule
15.00 & 1e-7 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 52.90 & 53.72 & 54.21 & 53.53 & 55.03 & 24.49 \\
15.00 & 1e-6 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 54.80 & 54.78 & 54.76 & 52.73 & 56.12 & 24.84 \\
15.00 & 1e-5 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 53.28 & 54.90 & 54.26 & 56.48 & 55.60 & 24.96 \\
15.00 & 1e-4 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 55.27 & 57.28 & 55.64 & 55.75 & 57.97 & 25.63 \\
15.00 & 1e-3 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 55.78 & 57.53 & 57.21 & 56.88 & 59.33 & 26.07 \\
15.00 & 1e-2 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 58.13 & 60.35 & 59.59 & 59.15 & 62.07 & 27.21 \\
15.00 & 0.10 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 61.95 & 62.48 & 63.50 & 63.95 & 67.78 & 29.06 \\
15.00 & 0.20 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 64.67 & 65.00 & 65.56 & 64.52 & 70.27 & 30.00 \\
15.00 & 0.40 & 0.00 & 0.00 & 21.86 & 0.00 & 0.00 & 20.35 & 66.25 & 69.23 & 69.03 & 66.90 & 74.27 & 35.26 \\
15.00 & 0.60 & 0.00 & 18.03 & 33.69 & 0.00 & 16.59 & 32.91 & 67.80 & 71.97 & 70.96 & 69.78 & 77.80 & 41.78 \\
15.00 & 0.80 & 18.00 & 31.12 & 49.75 & 14.04 & 28.11 & 46.88 & 70.48 & 74.10 & 74.24 & 72.33 & 79.65 & 50.79 \\
\midrule
N/A & N/A & 87.12 & 94.54 & 96.89 & 38.62 & 90.51 & 95.39 & 97.28 & 96.07 & 98.99 & 94.88 & 99.80 & 90.01 \\
\bottomrule
\end{tabular}


==> preamble/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> preamble/preamble.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%                               Preamble                                    %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% --- Draft flag (used in comments / markup if you want) ---------------------
% \usepackage{ifthen}
% \newcommand{\isdraft}{true}
% \newif\ifisdraft
% \isdrafttrue 
% \makeatletter
% \@ifundefined{ifisdraft}{\newif\ifisdraft}{}
% \isdrafttrue   % or \isdraftfalse
% \makeatother


% --- Encoding (pdfLaTeX default is utf8 now; harmless to keep) -------------
\usepackage[utf8]{inputenc}

% \usepackage{multibib}
% \newcites{A}{Appendix References} % defines \citeA, \bibliographyA, ...


% --- General utilities ------------------------------------------------------
\usepackage{microtype}
\usepackage{url}
\usepackage{xstring}     % used by appendix-only TOC helper below
\usepackage{comment}
\usepackage{textcomp}    % sometimes handy for symbols

% --- Graphics / figures -----------------------------------------------------
\usepackage{graphicx}    % CVPR loads this already; keeping is harmless
\usepackage{pgffor}      % for \foreach
\usepackage{wrapfig}     % wrap figures in text (do NOT nest floats inside)
\usepackage{float}
\usepackage{xparse} % once, in preamble
\NewDocumentCommand{\SubFig}{ O{} O{.48\linewidth} m }{%
  \begin{subfigure}[t]{#2}%
    #3%
    \caption{#1}%
  \end{subfigure}%
}



% --- Math -------------------------------------------------------------------
\usepackage{mathtools}   % extends amsmath (cvpr already loads amsmath)
\usepackage{xfrac}
\usepackage{amsthm}      % theorem environments

% --- Algorithms -------------------------------------------------------------
% \usepackage{algorithm}
% \usepackage{algorithmicx}
% \usepackage{algpseudocode}
% ---- algorithms: modern, ICML-safe
\usepackage{algorithm}        % float

% If legacy 'algorithmic' got loaded anywhere, neutralize it:
\usepackage{etoolbox}
\makeatletter
\@ifpackageloaded{algorithmic}{%
  \let\algorithmic\relax
  \let\endalgorithmic\relax
  \let\algorithmicrequire\relax
  \let\algorithmicensure\relax
  \let\algorithmiccomment\relax
  \let\ALG@beginalgorithmic\relax
  \let\ALG@endalgorithmic\relax
}{}
\makeatother

% Now load the modern stack that defines \begin{algorithmic}...\State etc.
\usepackage{algorithmicx}
\usepackage{algpseudocode}

% --- Tables / lists ---------------------------------------------------------
\usepackage{booktabs}    % CVPR loads this too; fine to keep
\usepackage{multirow}
\usepackage{enumitem}

% --- TikZ -------------------------------------------------------------------
\usepackage{tikz}
\usetikzlibrary{
  matrix,
  positioning,
  calc,
  decorations.pathreplacing,
  arrows.meta
}
\tikzset{
  cell/.style={draw,minimum width=6pt,minimum height=6pt,inner sep=0pt},
  grid/.style={gray!45,thin},
  font=\scriptsize
}

% Appendix-only table of contents via etoc tags (no global patching)
\usepackage{etoc}

\newcommand{\AppendixTOC}{%
  \section*{Appendix Contents}%
  \begingroup
    % Hide non-appendix entries; show appendix to chosen depth
    \etocsettagdepth{default}{none}%
    \etocsettagdepth{apx}{subsection}% change to subsubsection if you want
    \tableofcontents
  \endgroup
}


\usepackage{setspace}

\usepackage{dblfloatfix}
\usepackage{placeins}

% \newif\ifinappendix
% \pretocmd{\appendix}{\inappendixtrue}{}{}  % flag once we enter \appendix

% \makeatletter
% \let\APX@orig@addcontentsline\addcontentsline
% \renewcommand{\addcontentsline}[3]{%
%   \APX@orig@addcontentsline{#1}{#2}{#3}%
%   \ifinappendix
%     \ifstrequal{#2}{section}{\APX@orig@addcontentsline{apx}{section}{#3}}{%
%       \ifstrequal{#2}{subsection}{\APX@orig@addcontentsline{apx}{subsection}{#3}}{%
%         \ifstrequal{#2}{subsubsection}{\APX@orig@addcontentsline{apx}{subsubsection}{#3}}{}%
%       }%
%     }%
%   \fi
% }
% \newcommand{\appendixtableofcontents}{%
%   \section*{Appendix Contents}%
%   \@starttoc{apx}%
% }
% \makeatother
% --- Appendix-only table of contents support -----------------
% \usepackage{xstring}
% \usepackage{etoolbox}
% \newif\ifinappendix
% % Mark that we are in appendix as soon as \appendix is called
% \pretocmd{\appendix}{\inappendixtrue}{}{}

% \makeatletter
% % Delay our hook until *after* hyperref (and the class) patch \addcontentsline
% \AtBeginDocument{%
%   \let\APX@orig@addcontentsline\addcontentsline
%   \renewcommand{\addcontentsline}[3]{%
%     % always write the normal entry
%     \APX@orig@addcontentsline{##1}{##2}{##3}%
%     % if we are in appendix, also mirror section-like entries into .apx
%     \ifinappendix
%       \ifstrequal{##2}{section}
%         {\APX@orig@addcontentsline{apx}{section}{##3}}{%
%       \ifstrequal{##2}{subsection}
%         {\APX@orig@addcontentsline{apx}{subsection}{##3}}{%
%       \ifstrequal{##2}{subsubsection}
%         {\APX@orig@addcontentsline{apx}{subsubsection}{##3}}{}}}%
%     \fi
%   }%
% }



% --- Appendix-only table of contents (single safe patch) ---
% \usepackage{xstring,etoolbox}
% \newif\ifinappendix

% \makeatletter
% \AtBeginDocument{%
%   % flip the flag when \appendix is entered (works even if class redefines it)
%   \pretocmd{\appendix}{\inappendixtrue}{}{}%

%   % save the final \addcontentsline (after class/hyperref)
%   \let\APX@orig@addcontentsline\addcontentsline

%   % mirror appendix section entries into jobname.apx
%   \renewcommand{\addcontentsline}[3]{%
%     \APX@orig@addcontentsline{##1}{##2}{##3}%
%     \ifinappendix
%       \IfStrEq{##2}{section}{%
%         \APX@orig@addcontentsline{apx}{section}{##3}%
%       }{}%
%       \IfStrEq{##2}{subsection}{%
%         \APX@orig@addcontentsline{apx}{subsection}{##3}%
%       }{}%
%       \IfStrEq{##2}{subsubsection}{%
%         \APX@orig@addcontentsline{apx}{subsubsection}{##3}%
%       }{}%
%     \fi
%   }%
% }

% print the appendix-only ToC (avoid recursion while reading .apx)
% \newcommand{\appendixtableofcontents}{%
%   \section*{Appendix Contents}%
%   \begingroup
%     \let\addcontentsline\APX@orig@addcontentsline
%     \@starttoc{apx}%
%   \endgroup
% }
% \makeatother






% --- Theorem-like environments ---------------------------------------------
\theoremstyle{plain}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}

\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{assumption}[theorem]{Assumption}

\theoremstyle{remark}
\newtheorem{remark}[theorem]{Remark}



% \usepackage{flushend} % in the preamble





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%                             End Preamble                                  %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%








%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% %% %% %% Preamble File %% %% %% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% % Recommended, but optional, packages for figures and better typesetting: \usepackage{microtype} \usepackage{graphicx} % \usepackage{subcaption} \usepackage{subfigure} \usepackage{pgffor} % for \foreach (or \usepackage{tikz}) % \usepackage{subfig} \usepackage{booktabs} % for professional tables % \usepackage{hyperref} % \hypersetup{ % colorlinks = true, % linkcolor = {red!50!black}, % citecolor = {blue!50!black}, % urlcolor = {black} % } \usepackage{url} \usepackage{xstring} %% Draft Flag \newcommand{\isdraft}{true} % Attempt to make hyperref and algorithmic work together better: % \newcommand{\theHalgorithm}{\arabic{algorithm}} \usepackage{wrapfig} % For theorems and such \usepackage{amsmath} \usepackage{amssymb} \usepackage{mathtools} \usepackage{amsthm} \usepackage{xfrac} \usepackage{enumitem} % For the algorithm \usepackage{algorithm} % \usepackage{algorithmic} % note : algorithmic and algpseudocode are incompatible \usepackage{algorithmicx} \usepackage{algpseudocode} % \newcommand{\theHalgorithm}{\arabic{algorithm}} \usepackage{comment} \usepackage{multirow} % ---------- TikZ & libraries ---------- \usepackage{tikz} \usetikzlibrary{ matrix, % matrix of nodes positioning, % node positioning (above=of …) calc, % coordinate calculations decorations.pathreplacing, % braces arrows.meta % arrow tips } % ------------------------------------------------------------ % ---------- Styles ---------- \tikzset{ cell/.style={draw,minimum width=6pt,minimum height=6pt,inner sep=0pt}, grid/.style={gray!45,thin}, font=\scriptsize % global TikZ font } % if you use cleveref.. \usepackage[capitalize,noabbrev]{cleveref} %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% % THEOREMS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% \theoremstyle{plain} \newtheorem{theorem}{Theorem}[section] \newtheorem{proposition}[theorem]{Proposition} \newtheorem{lemma}[theorem]{Lemma} \newtheorem{corollary}[theorem]{Corollary} \theoremstyle{definition} \newtheorem{definition}[theorem]{Definition} \newtheorem{assumption}[theorem]{Assumption} \theoremstyle{remark} \newtheorem{remark}[theorem]{Remark} % Todonotes is useful during development; simply uncomment the next line % and comment out the line below the next line to turn off comments %\usepackage[disable,textsize=tiny]{todonotes} \usepackage[textsize=tiny]{todonotes} % \usepackage{hyperref} % \hypersetup{ % colorlinks = true, % linkcolor = {red!50!black}, % citecolor = {blue!50!black}, % urlcolor = {black} % } \usepackage{cleveref} % Smart cross-referencing \usepackage{etoc} % for local ToC % \etockeeporiginaltableofcontents % Make sure ToC depth & numbering are not suppressed % \setcounter{tocdepth}{2} % show down to \subsection % \setcounter{secnumdepth}{3} % number down to \subsubsection (safe) % --- Appendix-only ToC: mirror ToC entries while in the appendix --- \usepackage{etoolbox} \newif\ifinappendix \pretocmd{\appendix}{\inappendixtrue}{}{} % flag once we enter \appendix \makeatletter % Save the original \addcontentsline (hyperref's version, if loaded) \let\APX@orig@addcontentsline\addcontentsline % While in the appendix, clone section/sub(section) entries to jobname.apx \renewcommand{\addcontentsline}[3]{% \APX@orig@addcontentsline{#1}{#2}{#3}% \ifinappendix \ifstrequal{#2}{section}{\APX@orig@addcontentsline{apx}{section}{#3}}{% \ifstrequal{#2}{subsection}{\APX@orig@addcontentsline{apx}{subsection}{#3}}{% \ifstrequal{#2}{subsubsection}{\APX@orig@addcontentsline{apx}{subsubsection}{#3}}{}% }% }% \fi } % Command to print the appendix-only ToC \newcommand{\appendixtableofcontents}{% \section*{Appendix Contents}% \@starttoc{apx}% } \makeatother \usepackage{todonotes} \usepackage[utf8]{inputenc} % \usepackage{algorithm} % For the algorithm environment \usepackage{wrapfig} % For wrapping text around figures/algorithms




